Block Acceleration Without Momentum: On Optimal Stepsizes of Block Gradient Descent for Least-Squares

Block coordinate descent is a powerful algorithmic template suitable for big data optimization. This template admits a lot of variants including block gradient descent (BGD), which performs gradient descent on a selected block of variables, while keeping other variables fixed. For a very long time, the stepsize for each block has tacitly been set to one divided by the block-wise Lipschitz smoothness constant, imitating the vanilla stepsize rule for gradient descent (GD). However, such a choice for BGD has not yet been able to theoretically justify its empirical superiority over GD, as existing convergence rates for BGD have worse constants than GD in the deterministic cases. To discover such theoretical justification, we set up a simple environment where we consider BGD applied to least-squares with two blocks of variables. Assuming the data matrix corresponding to each block is orthogonal, we find optimal stepsizes of BGD in closed form, which provably lead to asymptotic convergence rates twice as fast as GD with Polyak's momentum; this means, under that orthogonality assumption, one can accelerate BGD by just tuning stepsizes and without adding any momentum. An application that satisfies this assumption is \textit{generalized alternating projection} between two subspaces, and applying our stepsizes to it improves the prior convergence rate that was once claimed, slightly inaccurately, to be optimal. The main proof idea is to minimize, in stepsize variables, the spectral radius of a matrix that controls convergence rates.

==> backup/ICLR-format/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%



\usepackage{amsfonts}
\usepackage{bm}
\usepackage{amsmath,amsthm,amssymb,rotating, mathrsfs}

\usepackage{mathtools}
\usepackage{cancel} 
\usepackage{xparse}
\usepackage{xfrac} % sfrac

% new command for mathcal
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathscr{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% new command for mathpzc
\newcommand{\pA}{\mathpzc{A}}
\newcommand{\pB}{\mathpzc{B}}
\newcommand{\pC}{\mathpzc{C}}
\newcommand{\pD}{\mathpzc{D}}
\newcommand{\pE}{\mathpzc{E}}
\newcommand{\pF}{\mathpzc{F}}
\newcommand{\pG}{\mathpzc{G}}
\newcommand{\pH}{\mathpzc{H}}
\newcommand{\pI}{\mathpzc{I}}
\newcommand{\pJ}{\mathpzc{J}}
\newcommand{\pK}{\mathpzc{K}}
\newcommand{\pL}{\mathpzc{L}}
\newcommand{\pM}{\mathpzc{M}}
\newcommand{\pN}{\mathpzc{N}}
\newcommand{\pO}{\mathpzc{O}}
\newcommand{\pP}{\mathpzc{P}}
\newcommand{\pQ}{\mathpzc{Q}}
\newcommand{\pR}{\mathpzc{R}}
\newcommand{\pS}{\mathpzc{S}}
\newcommand{\pT}{\mathpzc{T}}
\newcommand{\pU}{\mathpzc{U}}
\newcommand{\pV}{\mathpzc{V}}
\newcommand{\pW}{\mathpzc{W}}
\newcommand{\pX}{\mathpzc{X}}
\newcommand{\pY}{\mathpzc{Y}}
\newcommand{\pZ}{\mathpzc{Z}}
\newcommand{\pLambda}{\mathsf{\Lambda}}


\newcommand{\pa}{\mathpzc{a}}
\newcommand{\pb}{\mathpzc{b}}
\newcommand{\pc}{\mathpzc{c}}
\newcommand{\pd}{\mathpzc{d}}
\newcommand{\pe}{\mathpzc{e}}
\newcommand{\pf}{\mathpzc{f}}
\newcommand{\pg}{\mathpzc{g}}
\newcommand{\ph}{\mathpzc{h}}
% \newcommand{\pi}{\mathpzc{I}}
\newcommand{\pj}{\mathpzc{j}}
\newcommand{\pk}{\mathpzc{k}}
\newcommand{\pl}{\mathpzc{l}}
% \newcommand{\pm}{\mathpzc{m}}
\newcommand{\pn}{\mathpzc{n}}
\newcommand{\po}{\mathpzc{o}}
\newcommand{\pp}{\mathpzc{p}}
\newcommand{\pq}{\mathpzc{q}}
\newcommand{\pr}{\mathpzc{r}}
\newcommand{\ps}{\mathpzc{s}}
\newcommand{\pt}{\mathpzc{t}}
\newcommand{\pu}{\mathpzc{u}}
\newcommand{\pv}{\mathpzc{v}}
\newcommand{\pw}{\mathpzc{w}}
\newcommand{\px}{\mathpzc{x}}
\newcommand{\py}{\mathpzc{y}}
\newcommand{\pz}{\mathpzc{z}}


% new command for mathbb
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%% LINEAR ALGEBRA
% bold math for matrices
\newcommand{\mat}[1]{{\bm{#1}}}

\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\btheta}{\bm{\theta}}
% \newcommand{\pD}{\bm{\Lambda}}

\newcommand{\bLambda}{\bm{\Lambda}}

\newcommand{\brmp}{\bm{\mathrm{p}}}
\newcommand{\brmq}{\bm{\mathrm{q}}}

\newcommand{\brmx}{\bm{\mathrm{x}}}
\newcommand{\brmy}{\bm{\mathrm{y}}}
\newcommand{\brmR}{\bm{\mathrm{R}}}

% bold math for vectors
\renewcommand{\vec}[1]{{\bm{#1}}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\by}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
%\newcommand{\bf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bm{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
%\newcommand{\bm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bzeta}{\bm{\zeta}}


\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\CK}[1]{{\color{purple}{#1}}}
\newcommand{\noteC}[1]{{\color{blue} \textbf{CK:} #1}}

\newcommand{\LP}[1]{{\color{violet}{#1}}}
\newcommand{\noteL}[1]{{\color{blue} \textbf{LP:} #1}}

\newcommand{\RV}[1]{{\color{blue}{#1}}}


\newcommand{\balpha}{\bm{\lambda}}

% linear algebra operations
% \NewDocumentCommand{\norm}{mG{2}}{\left\lVert#1\right\rVert_{#2}}
\NewDocumentCommand{\norm}{mG{2}}{\big\|#1\big\|_{#2}}
\NewDocumentCommand{\ang}{m}{\langle #1 \rangle}
%\DeclarePairedDelimiter\ang{\langle}{\rangle}
\NewDocumentCommand{\pinv}{m}{#1^\dagger}
\newcommand{\trans}{\top}
\newcommand{\trsp}[1]{#1^\trans}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\im}{im}




\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\SE}{SE}


\DeclareMathOperator*{\Trace}{trace}

% calculus
\NewDocumentCommand{\integral}{mmmm}{\int_{#1}^{#2}{#3}{\text{ d}#4}}


%% OTHER COMMANDS
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}



% \NewDocumentCommand{\seq}{mG{n}}{{#1}_1, \dots, {#1}_{#2}}
\NewDocumentCommand{\seqp}{mG{n}}{{#1}_1-\cdots+ {#1}_{#2}}
\NewDocumentCommand{\seqm}{mG{n}}{{#1}_1-\cdots- {#1}_{#2}}


% \NewDocumentCommand{\set}{m}{\{#1\}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\myparagraph}[1]{\noindent\textbf{#1.}}
\newcommand{\myparagraphit}[1]{\noindent\textit{#1.}}


\newcommand{\rL}{\widetilde{L}}

\newcommand{\oR}{\overline{R}}

\DeclareMathOperator{\rgrad}{\widetilde{\nabla}}
\DeclareMathOperator{\retr}{Retr}

\DeclareMathOperator{\proj}{Proj}

\DeclareMathOperator{\rsgrad}{\tilde{\nabla}_{\textnormal{s}}}
\DeclareMathOperator{\sgrad}{\nabla_{\textnormal{s}}}


\DeclareMathOperator{\rsdifferential}{\tilde{\partial}}
\DeclareMathOperator{\sdifferential}{\partial}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\prox}{prox}

%\newtheorem{theorem}{Theorem}%  meant for continuous numbers
%%\newtheorem{theorem}{Theorem}[section]% meant for sectionwise numbers
%% optional argument [theorem] produces theorem numbering sequence instead of independent numbers for Proposition
% \newtheorem{proposition}[theorem]{Proposition}% 


\newtheorem{theorem}{Theorem}
\newtheorem{axiom}{Axiom}
\newtheorem{prop}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}


\theoremstyle{remark}
\newtheorem{remark}{Remark}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem{exercise}{Exercise}
\newtheorem{assumption}{Assumption}



\newtheorem{problem}{Problem}



==> backup_SIOPT_template/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}


\usepackage{bm}
% \usepackage{amsmath,amsthm,amssymb,rotating, mathrsfs}

\usepackage{mathtools}
\usepackage{cancel} 
\usepackage{xparse}
\usepackage{xfrac} % sfrac

% new command for mathcal
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathscr{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}



% new command for mathbb
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%% LINEAR ALGEBRA
% bold math for matrices
\newcommand{\mat}[1]{{\bm{#1}}}

\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\btheta}{\bm{\theta}}
% \newcommand{\pD}{\bm{\Lambda}}

\newcommand{\bLambda}{\bm{\Lambda}}

\newcommand{\brmp}{\bm{\mathrm{p}}}
\newcommand{\brmq}{\bm{\mathrm{q}}}

\newcommand{\brmx}{\bm{\mathrm{x}}}
\newcommand{\brmy}{\bm{\mathrm{y}}}
\newcommand{\brmR}{\bm{\mathrm{R}}}

% bold math for vectors
\renewcommand{\vec}[1]{{\bm{#1}}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\by}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
%\newcommand{\bf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bm{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
%\newcommand{\bm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bzeta}{\bm{\zeta}}


\newcommand{\beps}{\bm{\epsilon}}
\newcommand{\CK}[1]{{\color{purple}{#1}}}
\newcommand{\noteC}[1]{{\color{blue} \textbf{CK:} #1}}

\newcommand{\LP}[1]{{\color{violet}{#1}}}
\newcommand{\noteL}[1]{{\color{blue} \textbf{LP:} #1}}

\newcommand{\RV}[1]{{\color{blue}{#1}}}


\newcommand{\balpha}{\bm{\lambda}}

% linear algebra operations
% \NewDocumentCommand{\norm}{mG{2}}{\left\lVert#1\right\rVert_{#2}}
\NewDocumentCommand{\norm}{mG{2}}{\big\|#1\big\|_{#2}}
\NewDocumentCommand{\ang}{m}{\langle #1 \rangle}
%\DeclarePairedDelimiter\ang{\langle}{\rangle}
\NewDocumentCommand{\pinv}{m}{#1^\dagger}
\newcommand{\trans}{\top}
\newcommand{\trsp}[1]{#1^\trans}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\im}{im}




\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\SE}{SE}


\DeclareMathOperator*{\Trace}{trace}

% calculus
\NewDocumentCommand{\integral}{mmmm}{\int_{#1}^{#2}{#3}{\text{ d}#4}}


%% OTHER COMMANDS
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}



% \NewDocumentCommand{\seq}{mG{n}}{{#1}_1, \dots, {#1}_{#2}}
\NewDocumentCommand{\seqp}{mG{n}}{{#1}_1-\cdots+ {#1}_{#2}}
\NewDocumentCommand{\seqm}{mG{n}}{{#1}_1-\cdots- {#1}_{#2}}


% \NewDocumentCommand{\set}{m}{\{#1\}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\myparagraph}[1]{\textit{#1.}}
\newcommand{\myparagraphit}[1]{\textit{#1.}}


\newcommand{\rL}{\widetilde{L}}

\newcommand{\oR}{\overline{R}}

\DeclareMathOperator{\rgrad}{\widetilde{\nabla}}
\DeclareMathOperator{\retr}{Retr}

\DeclareMathOperator{\proj}{Proj}

\DeclareMathOperator{\rsgrad}{\tilde{\nabla}_{\textnormal{s}}}
\DeclareMathOperator{\sgrad}{\nabla_{\textnormal{s}}}


\DeclareMathOperator{\rsdifferential}{\tilde{\partial}}
\DeclareMathOperator{\sdifferential}{\partial}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\prox}{prox}


% Used for creating new theorem and remark environments
% \newtheorem{theorem}{Theorem}
% \newtheorem{axiom}{Axiom}
% \newtheorem{prop}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{fact}{Fact}


% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{question}{Question}
% \newtheorem{exercise}{Exercise}
\newtheorem{assumption}{Assumption}

% \newtheorem{problem}{Problem}

\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow,rotating}
\usepackage{subcaption}
% \pdfstringdefDisableCommands{%
% 	\let\Cref\crtCref
% 	\let\cref\crtcref
% }
\crefformat{equation}{(#2#1#3)}

% Sets running headers as well as PDF title and authors
\headers{Block Acceleration Without Momentum}{L. Peng and W. Yin}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Block Acceleration Without Momentum: On Optimal Stepsizes of Block Gradient Descent\thanks{Submitted to the editors DATE. \funding{This work was funded by XXX.}}}

% Authors: full names plus addresses.
\author{
On-going work
%Liangzu Peng\thanks{Work done during internship at Alibaba Group (US), Damo Academy 
%  (\email{lpenn@seas.upenn.edu}).}
%\and Wotao Yin\thanks{Alibaba Group (US), Damo Academy
%  (\email{wotao.yin@alibaba-inc.com}).}
}

\usepackage{amsopn}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

